Matrix product state of multi-time correlations

For an interacting spatio-temporal lattice system we introduce a formal way of expressing multi-time correlation functions of local observables located at the same spatial point with a time state, i.e. a statistical distribution of configurations observed along a time lattice. Such a time state is defined with respect to a particular equilibrium state that is invariant under space and time translations. The concept is developed within the Rule 54 reversible cellular automaton, for which we explicitly construct a matrix product form of the time state, with matrices that act on the 3-dimensional auxiliary space. We use the matrix-product state to express equal-space time-dependent density-density correlation function, which, for special maximum-entropy values of equilibrium parameters, agrees with the previous results. Additionally, we obtain an explicit expression for the probabilities of observing all multi-time configurations, which enables us to study distributions of times between consecutive excitations and prove the absence of decoupling of timescales in the Rule 54 model.

==> LatticeGeometry.tex <==
\definecolor{full}{rgb}{0,0,0}
\definecolor{old}{rgb}{1,1,1}
\definecolor{updated}{rgb}{0.9,0.9,0.9}
\definecolor{border}{rgb}{0.5,0.5,0.5}
\begin{tikzpicture}
  \def\a{0.65}
  \def\b{6}
  \def\off{0.75}
  \newcommand\coloredrectangle[3]{
    \draw[thick,black,fill=#3] ({\a*(#1)},{\a*(#2-1)})  -- ({\a*(#1+1)},{\a*(#2)})  -- ({\a*(#1)},{\a*(#2+1)})  
    -- ({\a*(#1-1)},{\a*(#2)})  -- cycle;
  }
  \newcommand\nbrectangle[2]{
    \draw[very thin,dashed,border] ({\a*(#1)},{\a*(#2-1)})  -- ({\a*(#1+1)},{\a*(#2)})  -- ({\a*(#1)},{\a*(#2+1)})  
    -- ({\a*(#1-1)},{\a*(#2)})  -- cycle;
  }
  \newcommand\bsawup[2]{
    \nbrectangle{#1+0}{#2+0};
    \nbrectangle{#1+1}{#2+1};
    \nbrectangle{#1+2}{#2+0};
    \nbrectangle{#1+3}{#2+1};
  }
  \newcommand\bsawdown[2]{
    \nbrectangle{#1+0}{#2+0};
    \nbrectangle{#1+1}{#2-1};
    \nbrectangle{#1+2}{#2+0};
    \nbrectangle{#1+3}{#2-1};
  }
  \newcommand\sawup[6]{
    \coloredrectangle{#1+0}{#2+0}{#3};
    \coloredrectangle{#1+1}{#2+1}{#4};
    \coloredrectangle{#1+2}{#2+0}{#5};
    \coloredrectangle{#1+3}{#2+1}{#6};
  }
  \newcommand\sawdown[6]{
    \coloredrectangle{#1+0}{#2+0}{#3};
    \coloredrectangle{#1+1}{#2-1}{#4};
    \coloredrectangle{#1+2}{#2+0}{#5};
    \coloredrectangle{#1+3}{#2-1}{#6};
  }
  \newcommand\uplabels[6]{
    \node at ({\a*(#1)},{\a*(#2)}) {#3};
    \node at ({\a*(#1+1)},{\a*(#2+1)}) {#4};
    \node at ({\a*(#1+2)},{\a*(#2)}) {#5};
    \node at ({\a*(#1+3)},{\a*(#2+1)}) {#6};
  }
  \newcommand\downlabels[6]{
    \node at ({\a*(#1)},{\a*(#2)}) {#3};
    \node at ({\a*(#1+1)},{\a*(#2-1)}) {#4};
    \node at ({\a*(#1+2)},{\a*(#2)}) {#5};
    \node at ({\a*(#1+3)},{\a*(#2-1)}) {#6};
  }

  \bsawup{0}{-2};
  \sawup{0}{0}{old}{old}{old}{old};
  \uplabels{0}{0}{${\scriptstyle s_{x-1,t}}$}{${\scriptstyle s_{x,t}}$}{${\scriptstyle s_{x+1,t}}$}{${\scriptstyle s_{x+2,t}}$};

  \bsawup{\b}{0};
  \bsawup{\b}{-2};
  \sawdown{\b}{0}{old}{updated}{old}{updated};
  \downlabels{\b}{0}{${\scriptstyle s_{x-1,t+1}}$}{${\scriptstyle s_{x,t+1}}$}{${\scriptstyle s_{x+1,t+1}}$}{${\scriptstyle s_{x+2,t+1}}$};

  \bsawup{2*\b}{0};
  \sawup{2*\b}{-2}{updated}{updated}{updated}{updated};
  \uplabels{2*\b}{-2}{${\scriptstyle s_{x-1,t+2}}$}{${\scriptstyle s_{x,t+2}}$}{${\scriptstyle s_{x+1,t+2}}$}{${\scriptstyle s_{x+2,t+2}}$};
  \draw[->] ({3.5*\a+\off*\a},-0.5) -- ({\b*\a-\off*\a},{-0.5});
  \draw[->] ({\b*\a+3.5*\a+\off*\a},-0.5) -- ({2*\b*\a-\off*\a},{-0.5});
\end{tikzpicture}

